Scheduling with Probabilistic Per-Packet Real-Time Guarantee for URLLC

For ultra-reliable, low-latency communications (URLLC) applications such as mission-critical industrial control and extended reality (XR), it is important to ensure the communication quality of individual packets. Prior studies have considered Probabilistic Per-packet Real-time Communications (PPRC) guarantees for single-cell, single-channel networks, but they have not considered real-world complexities such as inter-cell interference in large-scale networks with multiple communication channels and heterogeneous real-time requirements. To fill the gap, we propose a real-time scheduling algorithm based on \emph{local-deadline-partition (LDP)}, and the LDP algorithm ensures PPRC guarantee for large-scale, multi-channel networks with heterogeneous real-time constraints. We also address the associated challenge of schedulability test. In particular, we propose the concept of \emph{feasible set}, identify a closed-form sufficient condition for the schedulability of PPRC traffic, and then propose an efficient distributed algorithm for the schedulability test. We numerically study the properties of the LDP algorithm and observe that it significantly improves the network capacity of URLLC, for instance, by a factor of 5-20 as compared with a typical method. Furthermore, the PPRC traffic supportable by the LDP algorithm is significantly higher than that of state-of-the-art comparison schemes. This demonstrates the potential of fine-grained scheduling algorithms for URLLC wireless systems regarding interference scenarios.

==> Notes.tex <==


Future work
    compare with Industry practice with static interference control 
        dividing frequency bands into three? 


TWC/ToN submission
    Related work 
        * XR & Rel. 18
        
        scheduling vs. URLLC 
        interference detrimental to URLLC? 
        ICIC 
        
        Tony August 2022 arxiv paper? 
        
    Update and cite LDP arxiv; 
        why new?:-(
    
    ?
    spell check 
    
    Suggested reviewrs 
        Guodong Zhao, Guodong.Zhao@glasgow.ac.uk, University of Glasgow
        Sharon Hu, shu@nd.edu, University of Notre Dame 
        Song Han, song.han@uconn.edu, University of Connecticut 
        I-Hong Hou, ihou@tamu.edu, Texas A&M University 
        Abusayeed Saifullah, saifullah@wayne.edu, Wayne State University
        Ravi Prakash, ravip@utdallas.edu, University of Texas - Dallas 
        Zheng Dong, dong@wayne.edu, Wayne State University 


JSAC submission
    Related work
        \cite{2021aoi} try to minimize the peak aoi violation probability.
        \cite{Kuo:minAOI-scheduling,2022aoi, Modiano:minAOI, Hou:minAOIScheduling} try to minimize summed aoi or average aoi.

    per-slot RB allocation: leverage channel diversity 
    xURLLC: predictable URLLC 


TWC submission 
    * I made some further refinement of Section IV-D as well as the proof of Theorem 7 to help readers better appreciate the logic of the presentation as well as the significance of the results. Please check and apply similar strategies in future paper writing. 
        Please check the comment(s) too. 
    
    * ArXiv TR upload & update TR pointer to ArXiv in paper 
    
    * Make sure the page limit of TWC is observed. 
        It seems that some key proofs can be kept in the submission, and make sure all the proofs in the TWC submission are either in text or appendix. 

    spell check
    ?
    

Linguistic issues:
    - check the difference between "each other" and "one another".
    - Book "Elements of Style" 
    - ISU CELT training & resources


Address RTAS'22 review:
    - DP vs Pfair-type etc: delay jitter, context switch, computation overhead, others?     proportionate? 
        multi-channel & Algorithm 1 
    - Approximation ratio bound 

    - Examples are for single-channel
    - The presentation can be simplified by preceding the formal definition by simple examples showingthe concept. For example Definition 2 is overformalized, and is more intuitive with the help of a simple example. In definition 3 please describe in text, what the 3 different cases cover.
    - The description of algorithm 1 can be complemented by rather presenting a diagram showing the distributed nature of the algorithm. A sequence diagram showing the interaction or consensus protocol between links is more helpful. What is unclear is how the priority is exchanged among different nodes. While each transmitter can set its priority, how does it know what is the priority of the undecided channel. How is this information exchanged ? On which channel ? In particular, how is this realized: "if i’s priority is higher than that of every other UNDECIDED and ACTIVE member of i, Mi", before transmission starts. 
    - Since the authors compare with multiprocessor scheduling it may be a good idea to mention that "X_i" is similar to the execution demand in classical real-time theory.
    - Since the authors say they extend the work in [29], they must clearly mention what is the novelty in this article, and what was already part of [29].
    - Unclear why the link needs to only co-ordinate with the other links in the 2-hop neighbourhood. The explanation is unclear.
    - The authors must clearly describe what the objective of each experiment is and describe the graphs in more details. The x and the y axis titles do not help in understanding the graphs. Can the authors simply present the y axis as a percentage: histogram showing what percentage of links have the following relative deadlines, for instance ? What does ratio to the number of links imply ?
    - Aspects like the consensus time are not explored in the experiments.
    
    - The physical meaning of a feasible set is not explained which make the following part of the paper hard to follow.
    
    - Please double-check and address other review comments too. 
    
    - Please check the references to make sure that all the references are well formatted. 
    
    - ?, spell check 
    
    - Writing & presentation course/training from https://cce.grad-college.iastate.edu/resources 
    


***
RTAS submission 
    Spell check 
    URL of anonymous TR 
    Update arXiv TR 

    
Post RTAS submission task:
    - Pay attention to good article writing, especially how good articles are written. Also consider participating in ISU training workshops/classes, and reading book(s) on good writing. 
        

Journal submission:
    TWC format, e.g., only author name shows up below title; as reference, see https://www.ece.iastate.edu/~hongwei/group/publications/PRKS-TWC.pdf 


***
IWQoS submission: https://iwqos2021.ieee-iwqos.org/authors/call-for-symposium-papers/ 
- 10pages, 10pt
- Move some content (e.g., proof) to Technical Report, and refer to it in the conference submission; use LaTex \ifthenelse command to do conditional compilation so that only one copy of files is maintained; see the example for Theorem; you can change the setting of "short" to be true or false in LDP.tex; 
- Both paper and Technical Report need to be double-blind
- Technical Report can be stored in Dropbox with URL shared in the conference submission; 


1/31 to-dos:
1) Please check comments and revisions of Theorem 4 as well as Algorithms 2 and 3; 
2) Please revise the presentation of Algorithms 2 and 3 so that each Statement ends with ";", to be consistent throughput the whole paper;


*** 
Writing tips/work-to-do:
    - Be very clear on what the specific take-messages of the paper is, and use those messages to guide the writing itself (including the emotion/appreciation you expect a reader to have while/after the paper); 
    
    - Learn the conditions under which a, an, the, and plurals of a noun is used; 
    
    - Writing a paper is not just to tell readers what we have learned (i.e., simply giving them our results), but, more importantly, to share our journey of exploration (e.g., thought process) that has taken us to the results we ended up with. So, it is important to write the paper in a way so that, as readers progress in reading the article, the thought process led by our paper will enable the readers to come up the solutions we ended up coming up with ourselves. That is, we want to write the paper so that a well-trained reader will be able to come up with our solution her-/himself by reading the text before we actually presented our solution in the paper. 
    
    - Read and practice the lessons from "Elements of Style". 


Zhibo to-do: 
    Self-reflection: 
        Theorem 3, proof, and example text thereafter 
        
    Section IV
        - LDP: change it so that a node does not occupy multiple channels in a single time slot unless all the other non-idle (i..e, having traffic) nodes in $M_i$ has also got an opportunity to transmit; 
            **** LDP Algorithm refinement: A node transmits the same packet over multiple channels only if there is no interferer? 
                * Potential new ways of defining real-time urgency? 
                * Pipelined, pre-computation of schedulability? 
               If infeasible, leveraging ideas such as [RaptorQ rateless coding!] to reduce overhead. 
            * In cellular networks, BS makes decisions for all the nodes in its cell. 
            
        * Properties of feasible set: being union of cliques (to add to Theorem 3)
            For Algorithms 2 & 3: How is the results of Theorem 3 used in the algorithm exactly? 
        * [Done] Approximation ratio: Formula (23): Can you derive a numerical lower bound for the approximation ratio? Difficult. 
    
    Section V:
        - need to use real-world URLLC traffic scenarios  
            more than time units; channel numbers; # of nodes? 
        - EDF-based scheduling? 
            parallel tx.: EDF is also optimal 
                - not optimal for one cell (if no parallel)? 
                - no control on jitter at all
        - Are there scenarios when LDP may perform much better than EDF and G-algorithm. Right now, the maximum improvement is only ~36\%, which may not be that impressive. 
            shorter deadline, fewer channels, interference?
            
        - Figure name: use names of semantics meaning, instead of Figure XXX; one benefit of LaTEX is so that we do not have to care about numbers. 
    
    * Edits: change from 
            "real time" to "real-time" as qualifier
            "one cell" to "single-cell" 
            "access point" to "base station" or "BS"
            
            Do not hard-code numbers in references, use \label{} and \ref{} commands; 


